Detecting and Reducing Bias in a High Stakes Domain

Gang-involved youth in cities such as Chicago sometimes post on social media to express their aggression towards rival gangs and previous research has demonstrated that a deep learning approach can predict aggression and loss in posts. To address the possibility of bias in this sensitive application, we developed an approach to systematically interpret the state of the art model. We found, surprisingly, that it frequently bases its predictions on stop words such as "a" or "on", an approach that could harm social media users who have no aggressive intentions. To tackle this bias, domain experts annotated the rationales, highlighting words that explain why a tweet is labeled as "aggression". These new annotations enable us to quantitatively measure how justified the model predictions are, and build models that drastically reduce bias. Our study shows that in high stake scenarios, accuracy alone cannot guarantee a good system and we need new evaluation methods.

==> oldintro.tex <==
Gang-involved youth in cities such as Chicago increasingly post about their experience on social media, often expressing grief when friends or family members are shot and killed. 
As their grief turns to anger, their posts sometimes turn to retribution and ultimately to plans for revenge, which might subsequently affect life in the real world \cite{patton2016sticks, patton2017tweets}.
To prevent potential violence, Natural Language Processing researchers have built automatic tools to help violence outreach workers in some communities to identify such possibilities and intervene to diffuse situations \cite{blevins2016automatically}. 
In a nutshell, they asked domain experts to annotate tweets and classify them into 3 categories: 
1) Aggression, including insults, threats, bragging, hypervigilance and challenges to authority;
2) Loss, including distress, sadness, loneliness and death;
3) Other. 
After acquiring the annotated labels, they frame this task as a standard 3-way text classification problem and evaluate the system using the standard macro F-score.
